Learning to Localize Reference Trajectories in Image-Space for Visual Navigation

We present LoTIS, a model for visual navigation that provides robot-agnostic image-space guidance by localizing a reference RGB trajectory in the robot's current view, without requiring camera calibration, poses, or robot-specific training. Instead of predicting actions tied to specific robots, we predict the image-space coordinates of the reference trajectory as they would appear in the robot's current view. This creates robot-agnostic visual guidance that easily integrates with local planning. Consequently, our model's predictions provide guidance zero-shot across diverse embodiments. By decoupling perception from action and learning to localize trajectory points rather than imitate behavioral priors, we enable a cross-trajectory training strategy for robustness to viewpoint and camera changes. We outperform state-of-the-art methods by 20-50 percentage points in success rate on conventional forward navigation, achieving 94-98% success rate across diverse sim and real environments. Furthermore, we achieve over 5x improvements on challenging tasks where baselines fail, such as backward traversal. The system is straightforward to use: we show how even a video from a phone camera directly enables different robots to navigate to any point on the trajectory. Videos, demo, and code are available at https://finnbusch.com/lotis.

==> figures/dataset_stats/ar_diff.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width={0.049},
    xlabel={Aspect Ratio Difference},
    ylabel={Count},
    title={Aspect Ratio Absolute Difference (mean: 0.50)},
    ymajorgrids=true,
    grid style={dashed,gray!30},
    enlarge x limits=0.05,
    ymin=0,
]
\addplot[fill=blue!70!black, draw=black] coordinates {
    (0.025,146)
    (0.074,155)
    (0.123,123)
    (0.172,138)
    (0.222,133)
    (0.271,104)
    (0.320,141)
    (0.369,97)
    (0.419,113)
    (0.468,107)
    (0.517,108)
    (0.566,82)
    (0.616,69)
    (0.665,80)
    (0.714,82)
    (0.764,72)
    (0.813,59)
    (0.862,74)
    (0.911,75)
    (0.961,57)
    (1.010,51)
    (1.059,45)
    (1.108,44)
    (1.158,34)
    (1.207,27)
    (1.256,29)
    (1.305,19)
    (1.355,10)
    (1.404,3)
    (1.453,3)
};
\end{axis}
\end{tikzpicture}

==> figures/dataset_stats/fov_diff.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width={1.990},
    xlabel={FOV Difference (degrees)},
    ylabel={Count},
    title={FOV Absolute Difference (mean: 20.8°)},
    ymajorgrids=true,
    grid style={dashed,gray!30},
    enlarge x limits=0.05,
    ymin=0,
]
\addplot[fill=blue!70!black, draw=black] coordinates {
    (1.005,130)
    (2.996,154)
    (4.986,149)
    (6.976,137)
    (8.966,127)
    (10.956,113)
    (12.946,117)
    (14.936,109)
    (16.927,81)
    (18.917,95)
    (20.907,90)
    (22.897,80)
    (24.887,86)
    (26.877,97)
    (28.867,76)
    (30.858,73)
    (32.848,79)
    (34.838,57)
    (36.828,58)
    (38.818,60)
    (40.808,52)
    (42.798,58)
    (44.789,44)
    (46.779,39)
    (48.769,33)
    (50.759,26)
    (52.749,31)
    (54.739,12)
    (56.729,8)
    (58.720,9)
};
\end{axis}
\end{tikzpicture}

==> figures/dataset_stats/height_diff.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width={0.043},
    xlabel={Height Difference (m)},
    ylabel={Count},
    title={Height Absolute Difference (mean: 0.45m)},
    ymajorgrids=true,
    grid style={dashed,gray!30},
    enlarge x limits=0.05,
    ymin=0,
]
\addplot[fill=blue!70!black, draw=black] coordinates {
    (0.022,148)
    (0.065,144)
    (0.108,141)
    (0.151,137)
    (0.194,127)
    (0.237,108)
    (0.280,103)
    (0.323,101)
    (0.366,108)
    (0.409,86)
    (0.452,99)
    (0.495,97)
    (0.538,93)
    (0.581,89)
    (0.624,89)
    (0.667,64)
    (0.710,55)
    (0.753,77)
    (0.796,60)
    (0.839,53)
    (0.882,58)
    (0.925,49)
    (0.968,49)
    (1.011,34)
    (1.054,33)
    (1.097,18)
    (1.140,26)
    (1.183,15)
    (1.226,14)
    (1.269,5)
};
\end{axis}
\end{tikzpicture}

==> figures/dataset_stats/off_traj_dist.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=\textwidth,
    height=4cm,
    ybar,
    bar width={0.157},
    xlabel={Distance to Trajectory (m)},
    ylabel={Count},
    title={Off-Trajectory Distance (mean: 2.81m)},
    ymajorgrids=true,
    grid style={dashed,gray!30},
    enlarge x limits=0.05,
    ymin=0,
]
\addplot[fill=blue!70!black, draw=black] coordinates {
    (1.580,84)
    (1.737,55)
    (1.893,43)
    (2.050,74)
    (2.206,54)
    (2.363,57)
    (2.519,35)
    (2.676,56)
    (2.832,29)
    (2.989,57)
    (3.145,28)
    (3.302,21)
    (3.459,14)
    (3.615,14)
    (3.772,7)
    (3.928,15)
    (4.085,12)
    (4.241,14)
    (4.398,13)
    (4.554,13)
    (4.711,11)
    (4.867,7)
    (5.024,4)
    (5.180,9)
    (5.337,3)
    (5.493,6)
    (5.650,6)
    (5.806,2)
    (5.963,4)
    (6.120,2)
    (6.276,0)
    (6.433,1)
    (6.589,1)
    (6.746,2)
    (6.902,2)
    (7.059,0)
    (7.215,0)
    (7.372,1)
    (7.528,0)
    (7.685,0)
    (7.841,1)
    (7.998,1)
    (8.154,0)
    (8.311,0)
    (8.468,0)
    (8.624,1)
    (8.781,0)
    (8.937,0)
    (9.094,0)
    (9.250,1)
};
\end{axis}
\end{tikzpicture}
